A Simple Methodology for Computing Families of Algorithms

Discovering "good" algorithms for an operation is often considered an art best left to experts. What if there is a simple methodology, an algorithm, for systematically deriving a family of algorithms as well as their cost analyses, so that the best algorithm can be chosen? We discuss such an approach for deriving loop-based algorithms. The example used to illustrate this methodology, evaluation of a polynomial, is itself simple yet the best algorithm that results is surprising to a non-expert: Horner's rule. We finish by discussing recent advances that make this approach highly practical for the domain of high-performance linear algebra software libraries.

==> WorksheetTemplate.tex <==
\renewcommand{\invariant}{{
		\colorbox{yellow!30}{$( \forall i ~\vert~ 0 \leq i <  k :   y(i) = \widehat y( i ) )$}
		\wedge	\colorbox{orange!30}{$
			( \forall i ~\vert~ k \leq i <  n :   y(i) = \widehat y(i) + x( i ))$} \wedge 0 \leq k \leq n } }

\renewcommand{\invariant}{}

\renewcommand{\loopguard}{{0<k}}

\renewcommand{\loopguard}{}

\begin{figure*}[p]
	\begin{Pseudocode}
		\renewcommand{\precondition}{$   0 \leq \size( b ) $}
	\renewcommand{\precondition}{}
	
	\PseudocodeAssert{}% $ Q: ( \forall i ~\vert~ 0 \leq i < n : y( i ) = \widehat y( i ) ) \wedge 0 \leq n$}
		\PseudocodeAssert{$ \wp( \leftdq S_I \rightdq, \PInv ):
			\phantom{\begin{array}[t]{@{}rcl}
			\begin{array}[b]{c}{
				\colorbox{yellow!50}{$
					( \forall i ~\vert~ 0 \leq i < 0 :  y(i) = \widehat y( i ) + x(i) )$} 
			} 
			\end{array}
			&\wedge&  
			\colorbox{yellow!50}{$( \forall i ~\vert~ 0 \leq i < n :  y(i) = \widehat y( i ) )$}  
			\\
			&\wedge&   0 \leq n \leq  n
			\end{array}}
			$}
		\PseudocodeStatement{$ \phantom{k:=n} $}
		\PseudocodeAssert{$ \PInv: \invariant $}
		\PseudocodeStatement{{\bf while} \phantom{$\loopguard$} {\bf do}} 
		\PseudocodeAssertIndent{$ \PInv \wedge G: $\\
			$\invariant \wedge$$ \phantom{\loopguard} \\
			 \phantom{\begin{array}[t]{rcl}
			\colorbox{yellow!50}{$( \forall i ~\vert~ 0 \leq i < k-1 :  y(i) = \widehat y( i ) + x(i) )$}
			&\wedge &
			\colorbox{blue!20}{$y(k-1) = \widehat y(k-1)$} \\
			\wedge 
			\colorbox{yellow!50}{$( \forall i ~\vert~ k \leq i < n :  y(i) = \widehat y( i ) + x(i) )$}  &\wedge&   0 < k \leq  n\\[0.3in]
			\end{array}}$}
		\PseudocodeAssertIndent{$\begin{array}{@{}l}
			\wp( \leftdq S_U; k := k-1 \rightdq, \PInv ):\\
			~~~~~~~~~~~~~~\phantom{\begin{array}[t]{rcl}
			\colorbox{yellow!50}{$( \forall i ~\vert~ 0 \leq i < k-1 :  y(i) = \widehat y( i ) )$}
			&\wedge &
			\colorbox{blue!20}{$y(k-1) + x(k-1) = \widehat y(k-1) + x(k-1)$} \\
			\wedge 
			\colorbox{yellow!50}{$( \forall i ~\vert~ k \leq i < n :  y(i) = \widehat y( i ) + x(i))$}  &\wedge&   0 \leq k-1 \leq  n\\[0.3in]
			\end{array}}
			\end{array}$}
		\PseudocodeStatementIndent{$ S_U: \phantom{y(k-1) := y(k-1) + x(k-1) } $}  
		\PseudocodeAssertIndent{$\begin{array}{@{}l}
			\wp( \leftdq k := k-1 \rightdq, \PInv):\\
			~~~~~~~~~~~~~~\phantom{\begin{array}[t]{rcl}
			\colorbox{yellow!50}{$( \forall i ~\vert~ 0 \leq i < k-1 :  y(i) = \widehat y( i ) )$}
			&\wedge &
			\colorbox{blue!20}{$y(k-1) = \widehat y(k-1) + x(k-1)$} \\
			\wedge 
			\colorbox{yellow!50}{$( \forall i ~\vert~ k \leq i < n :  y(i) = \widehat y( i ) + x(i))$}  &\wedge&   0 \leq k-1 \leq  n\\[0.3in]
			\end{array}}
			\end{array} $}
		\PseudocodeStatementIndent{$ k := k-1 $}  
\NoShow{		\PseudocodeAssertIndent{$\begin{array}{@{}l}
			\PInv:\\
			~~~~~~~~~~~~~~\phantom{\begin{array}[t]{rcl}
			\colorbox{yellow!50}{$( \forall i ~\vert~ 0 \leq i < k :  y(i) = \widehat y( i ) )$}
			&\wedge &
			\colorbox{blue!20}{$y(k) = \widehat y(k) + x(k)$} \\
			\wedge 
			\colorbox{yellow!50}{$( \forall i ~\vert~ k < i < n :  y(i) = \widehat y( i ) + x(i))$}  &\wedge&   0 \leq k \leq  n.
			\end{array}}
			\end{array} $}
		}
		\PseudocodeAssertIndent{$\PInv: \invariant $}	
		\PseudocodeStatement{{\bf endwhile}}
		\PseudocodeAssert{$ \PInv \wedge \neg G: \invariant$ $\wedge$ $ \neg ( \phantom{\loopguard} )$ }	
	\PseudocodeAssert{}% $R: ( \forall i ~\vert~ 0 \leq i < n :  y(i) = \widehat y( i ) + x( i )) $}
	\end{Pseudocode}
	
	\caption{Blank worksheet for adding vector $ x $ to vector $ y $ (Variant 2).}
	\label{fig:BlankVariantTwo}
\end{figure*}
